Not All or None: Dynamic Construction of Target-aware Memory Graph for Conversational Stance Detection

Stance detection is crucial for understanding the underlying attitude of an expression towards a target. Conversational stance detection is a more challenging stance detection task in real-world social media scenarios, as it involves detecting the user's stance by leveraging the target-related historical statements across conversational sessions. In this paper, we propose target-aware Memory Graph TamGraph, a novel method that dynamically leverages target-related statements for conversational stance detection. Instead of considering all preceding historical conversations or using no prior conversation information for stance detection, our TamGraph employs a stepwise, entropy-guided backtracking mechanism to selectively activate memory from historical conversations and dynamically constructs a target-aware graph to model the stance relations among utterances. This allows the exploitation of target-related information from the conversation history for stance detection while preventing the introduction of noise. Experimental results on both English and Chinese benchmarks demonstrate that our TamGraph substantially improves LLM performance on conversational stance detection.

==> sections/Biases.tex <==
\section{Biases of LLMs in Conversational Stance Detection} 
\label{sec:Biases}
We conduct experiments on two benchmarks. For English, we use MT-CSD \cite{niu-etal-2024-challenge}, which contains 15876 instances with Bitcoin, Tesla, SpaceX, Biden, and Trump as targets. For Chinese, we use ZS-CSD \cite{ding-etal-2025-zero}, which consists of 17063 conversations with 113 noun-phrase-type targets and 167 claim-type targets. Their labels are either favor, against or none. \par
For models, we evaluate six LLMs of various sizes: Qwen2.5-Instruct (3B, 7B, 14B) \cite{qwen2.5}, Qwen3-4B-Instruct-2507 \cite{yang2025qwen3}, Llama-3.1-8B-Instruct \cite{grattafiori2024llama}, and GPT-4o-mini \cite{achiam2023gpt}. All models are evaluated on MT-CSD. On ZS-CSD, we exclude Llama-3.1-8B-Instruct due to its limited native support for Chinese.\par
We consider two input settings: (i) \emph{single-turn input}, where LLMs only receive the target utterance, and (ii) \emph{multi-turn input}, where LLMs also receive the entire conversation. Since stance detection requires stable predictions, and to ensure reproducibility, we set the temperature to 0. For MT-CSD, we design prompts in English, whereas for ZS-CSD we use their Chinese translations to remain consistent with the its native languages. The prompts are detailed in the Table \ref{tab:prompt_single_input} and Table \ref{tab:prompt_multi_input} in the section \ref{sec:prompts} in the Appendix. Model performance is evaluated using accuracy and macro F1.\par
For MT-CSD, we treat each combination of a target and a model as one group. Since ZS-CSD is not pre-partitioned by target, we regard each model as one group. Therefore, we raise the question: \emph{does multi-turn input consistently outperform single-turn input in the same group?} \par
Table~\ref{tab:single-multi comparision} presents the results, and the answer is clearly ``\textbf{No}''. Among the 35 groups, the single-turn input achieves higher accuracy in 15 cases and higher macro F1 in 14 cases. From these results, we draw two observations: (i) although multi-turn input often boosts performance, there is a non-negligible number of cases where it actually degrades performance for certain models and targets; and (ii) the benefit of multi-turn input is highly model- and target-dependent, indicating that additional turns is not uniformly advantageous for LLM-based stance detection.

\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Model} &
\multicolumn{5}{c}{MT-CSD (acc. / F1 in \%)} &
\multirow{2}{*}{\begin{tabular}{@{}c@{}}ZS-CSD\\(acc. / F1 in \%)\end{tabular}} \\
\cmidrule(lr){2-6}
& Bitcoin & Tesla & SpaceX & Biden & Trump & \\
\midrule
GPT-4o-mini (single)
& 49.07/48.33 & 71.48/67.73 & 61.99/59.38 & 44.28/34.61 & 66.49/53.72
& 43.65/38.94 \\

\rowcolor{gray!20}
GPT-4o-mini (multi)
& \textcolor{blue}{53.53}/\textcolor{blue}{53.48}
& \textcolor{red}{69.26}/\textcolor{red}{62.61}
& \textcolor{blue}{66.67}/\textcolor{blue}{64.86}
& \textcolor{blue}{48.18}/\textcolor{blue}{39.96}
& \textcolor{blue}{68.81}/\textcolor{red}{51.96}
& \textcolor{blue}{45.99}/\textcolor{blue}{42.70} \\

\midrule
Qwen2.5-3B (single)
& 47.03/42.96 & 47.22/43.78 & 46.11/46.77 & 31.39/30.02 & 48.84/34.43
& 33.55/25.53 \\

\rowcolor{gray!20}
Qwen2.5-3B (multi)
& \textcolor{blue}{48.69}/\textcolor{blue}{43.80}
& \textcolor{red}{37.41}/\textcolor{red}{35.26}
& \textcolor{red}{41.74}/\textcolor{red}{40.98}
& \textcolor{blue}{34.31}/\textcolor{blue}{34.69}
& \textcolor{red}{38.15}/\textcolor{red}{28.49}
& \textcolor{red}{31.11}/\textcolor{red}{20.77} \\

\midrule
Qwen2.5-7B (single)
& 44.98/42.32 & 70.91/58.24 & 64.17/57.37 & 45.74/31.76 & 66.67/51.15
& 39.43/28.53 \\

\rowcolor{gray!20}
Qwen2.5-7B (multi)
& \textcolor{blue}{50.00}/\textcolor{blue}{49.24}
& \textcolor{red}{66.11}/\textcolor{red}{57.33}
& \textcolor{red}{63.24}/\textcolor{blue}{58.50}
& 45.74/\textcolor{blue}{36.68}
& \textcolor{blue}{69.16}/\textcolor{red}{46.71}
& \textcolor{blue}{39.63}/\textcolor{blue}{31.45} \\

\midrule
Qwen2.5-14B (single)
& 46.65/46.09 & 66.67/59.68 & 63.86/61.25 & 42.82/33.86 & 59.18/42.10
& 46.32/43.96 \\

\rowcolor{gray!20}
Qwen2.5-14B (multi)
& \textcolor{blue}{54.09}/\textcolor{blue}{51.19}
& \textcolor{red}{50.00}/\textcolor{red}{45.67}
& \textcolor{red}{53.89}/\textcolor{red}{53.62}
& \textcolor{red}{41.85}/\textcolor{blue}{41.60}
& \textcolor{red}{49.38}/\textcolor{red}{39.10}
& \textcolor{red}{45.09}/\textcolor{blue}{44.00} \\

\midrule
Qwen3-4B-2507 (single)
& 43.87/42.97 & 69.63/59.52 & 69.16/62.31 & 46.47/28.93 & 67.91/51.09
& 39.20/34.72 \\

\rowcolor{gray!20}
Qwen3-4B-2507 (multi)
& \textcolor{blue}{44.61}/\textcolor{blue}{44.69}
& \textcolor{red}{57.96}/\textcolor{red}{53.17}
& \textcolor{red}{58.57}/\textcolor{red}{55.30}
& \textcolor{blue}{54.74}/\textcolor{blue}{48.96}
& \textcolor{red}{59.54}/\textcolor{red}{46.53}
& \textcolor{blue}{39.67}/\textcolor{blue}{36.60} \\

\midrule
Llama-3.1-8B (single)
& 36.99/34.21 & 39.81/37.71 & 44.86/41.71 & 44.04/33.57 & 40.64/36.15
& --- \\

\rowcolor{gray!20}
Llama-3.1-8B (multi)
& \textcolor{blue}{49.81}/\textcolor{blue}{49.51}
& \textcolor{blue}{58.70}/\textcolor{blue}{52.23}
& \textcolor{blue}{58.88}/\textcolor{blue}{56.78}
& \textcolor{blue}{50.85}/\textcolor{blue}{43.80}
& \textcolor{blue}{41.35}/\textcolor{blue}{37.13}
& --- \\
\bottomrule
\end{tabular}
\caption{Comparison of single-turn vs.\ multi-turn inputs for LLMs on MT-CSD and ZS-CSD. Values in \textcolor{blue}{blue} indicate that the multi-turn input outperforms the single-turn input, while values in \textcolor{red}{red} indicate a performance drop.}
\label{tab:single-multi comparision}
\end{table*}


To further understand the observations, we additionally analyse (i) \emph{conversational stance bias} and (ii) \emph{conversational relevance bias}.\par
\paragraph{Conversational stance bias.}
For each instance \(i\) in a group \(g\), \(y_i\) denote the ground truth, \(y_i^{\text{multi}}\) is the model’s prediction for the target utterance under multi-turn input, and \(y_i^{\text{dlg}}\) is the stance the same model assigns to the entire conversation. We partition instances into:
\begin{equation}
\mathcal{C}_g = \{ i \mid y_i^{\text{multi}} = y_i \},
\mathcal{E}_g = \{ i \mid y_i^{\text{multi}} \neq y_i \}
\end{equation}
corresponding to correct and error cases.\par
We define the alignment on correct cases \(A^{\text{correct}}_g\), alignment on errors \(A^{\text{error}}_g\) and Bias index \(B_g\) as:
\begin{equation}
A^{\text{correct}}_g
= \frac{1}{|\mathcal{C}_g|} \sum_{i \in \mathcal{C}_g}
\mathbf{1}\big[ y_i^{\text{multi}} = y_i^{\text{dlg}} \big],
\end{equation}

\begin{equation}
A^{\text{error}}_g
= \frac{1}{|\mathcal{E}_g|} \sum_{i \in \mathcal{E}_g}
\mathbf{1}\big[ y_i^{\text{multi}} = y_i^{\text{dlg}} \big],
\end{equation}

\begin{equation}
B_g = A^{\text{error}}_g - A^{\text{correct}}_g,
\end{equation}

which measure the alignment between \(y_i^{\text{multi}}\) and \(y_i^{\text{dlg}}\)  for correct and error cases, respectively. \(B_g\) reflects the extent to which errors are more aligned with the entire-conversation stance than correctness.
\par

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/biases.pdf}
    \caption{conversation stance bias. }
    \label{fig:biases}
\end{figure}

We report \(A^{\text{correct}}_g\) and \(A^{\text{error}}_g\), averaged over three subsets of groups: (i) \(G_B\), where multi-turn input boosts performance, (ii) \(G_D\), where it degrades performance, and (iii) all groups, for the two benchmarks separately. Figure~\ref{fig:biases} shows the results. Across all subsets, \(A^{\text{error}}_g\) is consistently higher than \(A^{\text{correct}}_g\), and \(G_D\) has larger \(B_g\) than \(G_B\), indicating a stronger conversation stance bias. Thus, additional turns in the conversation do not merely offer extra evidence, instead, their global stance impose a harmful bias on the detection on the target utterance.\par

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}{*}{} &
\multicolumn{5}{c}{MT-CSD} &
\multirow{2}{*}{ZS-CSD} \\
\cmidrule(lr){2-6}
& Bitcoin & Tesla & SpaceX & Biden & Trump & \\
\midrule
Irr.
& 27.64 & 22.21 & 17.03 & 60.89 & 24.69 & 56.51 \\
\bottomrule
\end{tabular}
\caption{conversation relevance bias.}
\label{tab:irrelevance-rate}
\end{table}

\paragraph{Conversational relevance bias.}
We further examine the percentage of the irrelevant utterances in the conversations in the two benchmarks respectively. Specifically, we adopt GPT-4o-mini as the evaluator to classify each utterance in conversations as either relevant or irrelevant to the given target (The prompts are detailed in the Table \ref{tab:prompt_relevance} in the section \ref{sec:prompts} in the Appendix), and compute the \emph{irrelevance rate} as the proportion of utterances labelled as irrelevant. Table \ref{tab:irrelevance-rate} shows the results, which indicates that a non-negligible number of turns do not contribute target-related evidence. \par
Overall, together with the conversational stance bias, these findings suggest that additional turns in conversations can introduce misleading and target-irrelevant content, which disrupt the LLM’s stance detection for the target utterance.

